State Machine Mutation-based Testing Framework for Wireless Communication Protocols

This paper proposes Proteus, a protocol state machine, property-guided, and budget-aware automated testing approach for discovering logical vulnerabilities in wireless protocol implementations. Proteus maintains its budget awareness by generating test cases (i.e., each being a sequence of protocol messages) that are not only meaningful (i.e., the test case mostly follows the desirable protocol flow except for some controlled deviations) but also have a high probability of violating the desirable properties. To demonstrate its effectiveness, we evaluated Proteus in two different protocol implementations, namely 4G LTE and BLE, across 23 consumer devices (11 for 4G LTE and 12 for BLE). Proteus discovered 25 unique issues, including 112 instances. Affected vendors have positively acknowledged 14 vulnerabilities through 5 CVEs.

==> sections/7_tracebuilder_02_works.tex <==
\section{\dpalgo: Generating Test Cases from Test Skeletons and Guiding PSM}
\label{sec:tracebuilder}
Given a test skeleton \tracesup{a} representing violations of a security property $\phi \in \Phi$ and a guiding PSM $\mathcal{M}$, \system mutates $\mathcal{M}$ 
%, a mutation budget $\mu$ and a length budget $\lambda$, 
to efficiently generate meaningful test cases \tracesup{c} with the shape of \tracesup{a}. We now discuss 
%how we use an existing technique to automatically extract PSM from protocol specifications. We then illustrate 
our PSM mutation strategies, and  
% $\mathcal{M}$ 
% tailored for testing protocol implementations. We 
then present our test case generation mechanism.  %that takes into account the test skeleton(s), $\mathcal{M}$, mutation budget $\mu$ and length budget $l$ to construct effective traces. 


%construction technique to automatically we formulate a dynamic programming algorithm. Formally, the dynamic programming problem is formulated as follows.
\begin{comment}
\subsection{Constructing a Guiding PSM}
\todo{Modify}
% \ishtiaq{in my opinion, we need a subsection before this one that discusses alphabet and scope. based on that, we can write PSM construction. Without knowing the scope/alphabet, it is not possible to define/extract the PSM.}

%\system requires a guiding PSM as input to generate test traces. 
To construct a guiding PSM for a black-box protocol implementation, one can infer the PSM using black-box automata learning \cite{dikeue, blediff} \citereq through input/output observations or extract the PSM from the protocol specification. Since automata learning is prohibitively expensive and PSM construction is not the main focus of this paper, we leverage an existing natural language processing (NLP)-based technique, Hermes \cite{hermes}, to extract an PSM from protocol specifications. 

% \syed{Summarize the workflow of HERMES in one paragraph here.} \mukit{@Ishtiaq}
Hermes, at first, takes natural language specifications and 
uses a neural constituency parsing technique to identify transition components, e.g., conditions, actions, and states.
For instance, in the text, ``Upon receipt of the IDENTITY REQUEST message, the UE shall send an IDENTITY RESPONSE message to the network,'' Hermes marks ``Upon receipt \dots{} message'' as the condition and ``the UE shall \dots{} network'' as the action.
It then generates a logical formula for each component using a rule-based approach, leveraging a deep learning-based dependency parser and a domain-specific language. 
For the same example, ``the UE shall \dots{} network'' is translated to ``$\mathsf{channel\_ue\_to\_mme} = \mathsf{identity\_response}$.''
After that, these formulas for different transition components are then compiled into transitions.
Hermes then assembles all generated transitions, checks for inconsistencies, and finally constructs a finite state machine for the system. 

% It then translates each transition component to logical formulas and finally compiles them into an PSM. 
% As discussed in \todo{REF}, we first define our scope and alphabet.
% Then, according to the scope and the defined alphabet,
% we provide natural language specifications to Hermes to extract the PSMs. 
% Further, the Hermes-extracted PSM relies on many internal state variables as well as input messages to make transitions. 
% On the other hand, as a black box testing framework, \system needs an PSM with an observational form, i.e., transitions with input and output messages. 
% Thus, we leverage UEGEN from Hermes to convert the extracted PSM to the required observational form. 
% of PSM, which demonstrates the output of the device under test upon receiving different inputs in different states.
% \ishtiaq{please take a look if ``observational form'' makes sense.}

The PSMs generated by HERMES may contain some incorrect transitions, i.e., wrong source or destination state, or wrong conditions (i.e., inputs) or actions (outputs) of a transition.  
To tackle this, \system{}'s technique of incorporating test skeletons and mutations into test generation does not necessarily require an error-free guiding PSM for testing. However, the accuracy of the guiding PSM impacts its efficiency in detecting vulnerabilities, as we demonstrate through an experiment provided in Section \todo{\textbf{[REF]}}. 

%Additionally, \system requires an input and output alphabet consisting of message types and their associated predicates. Hermes not only provides a detailed PSM from the specifications but also provides a set of messages and predicates (e.g., different fields and their values). We construct the input and output alphabet of \system by utilizing the extracted set of messages and predicates from Hermes.
\end{comment}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/mutation_example_ccs_v1.pdf}
%     \caption{Example of Mutations on guiding PSM. The original PSM is shown in Figure \ref{fig:ble_running_example}. The red transitions are the mutated transitions.
%     }
%     \label{fig:mutation_example}
% \end{figure}

\begin{comment}
    \subsection{Mutating a PSM}
\label{sec:tracebuilder:mutation}
As discussed in challenge \textbf{C3} in \todo{Section~\ref{sec:design_challenges}}, since the guiding PSM is assumed to satisfy all security properties, we need to mutate the guiding PSM $\mathcal{M}$, i.e., PSM transitions to generate traces satisfying the regular expression \tracesup{a}, which signifies the violation of a security property. 
To perform mutation over a given transition $\mathcal{R}(q_c, \alpha, \beta, q_n)$, 
%where $q_c$ and $q_n$ are source and destination states, and $\alpha$ and $\beta$ are input and output of that transition, respectively, 
\system primarily performs two types of mutations:  (\textbf{M1}) mutation over the observation of a transition to trigger the input/output observation ${(\alpha, \beta)}_m$, and (\textbf{M2}) mutation over the destination state of a transition $q_n$, leading to a destination state $q_m \in \mathcal{Q} (q_m \neq q_n)$. 

Mutation type \textbf{M1} leads to the generation of traces where a mutated version of input message $\alpha$ is tested when the target implementation $\mathcal{I}_{P}$ reaches state $q_c$, with the hope of triggering a security property violation or a deviation (a behavior different from what the guiding PSM suggests). For this kind of mutation, \system randomly applies one perturbation from a %\textit{mutation pool}, which is 
a pool of mutation strategies. For example, it replaces an integrity-protected message with a plaintext or a replayed one, or varies security-sensitive fields (e.g., in LTE, security header type, identity type in identity request message) in messages, and their combination thereof (e.g., plaintext identity request with identity type 3 (TMSI) and security header type 1).


Mutation type \textbf{M2} generates a trace that tests whether input message $\alpha$ at state $q_c$ leads to a state $q_m$ different than what is expected (in this case $q_n$) by the guiding PSM, which in turn can lead to an observable deviation or security property violation. This kind of mutation also enables \system to detect certain bypass attacks. For example, the logical flow of SC (Secure Connections) key pairing in BLE is \keyexchange, \smrandomsend, \dhkeycheck, \encreq. More specifically, if \system considers mutating the destination state of the key exchange message to the state for \dhkeycheck, \system can test whether bypassing \smrandomsend is possible.


As examples of mutation kinds \textbf{M1} and \textbf{M2}, consider the examples shown in Figure \ref{fig:mutation_example}. Suppose we are performing mutation over the transition $\mathcal{R}$($q_4$,\encpausereqbenignfull, \nullaction, $q_4$). As an example of mutation kind \textbf{M1}, we can perform mutation over the observation $a_{ep}$, and and test it with mutated observation ${(a_{ep})}_m$. A practical example of mutation over $a_{ep}$ could be testing with input \encpausereqreplay, which tests whether the target implementation properly handles the message at state $q_4$ or not. As an example of mutation kind \textbf{M2}, we can perform a mutation over the next state $q_4$ of the transition by changing the next state of the transition to $q_0$. This mutation would generate a trace that tests whether the target implementation incorrectly goes back to state $q_0$ if \encpausereqbenignfull is fed at state $q_4$.
\end{comment}

%\vspace{-2mm}
\subsection{Mutating a PSM}
\label{sec:tracebuilder:mutation}

As discussed in challenge \textbf{C2} in section~\ref{sec:overview_and_challenges}, since the guiding PSM is assumed to satisfy all security properties, we need to mutate the guiding PSM $\mathcal{M}$, i.e., PSM transitions to generate traces satisfying a test skeleton \tracesup{a}, which signifies the violation of a security property. \system selects a transition $\mathcal{R}(q_c, \alpha, \gamma, q_n)$ to mutate while generating concrete traces satisfying a test skeleton \tracesup{a} as described in detail in \S\ref{sec:tracebuilder:trace_generation}. 
%\textcolor{red}{Since this selection is based on the defined transitions in the guiding PSM and driven by the goal of satisfying a test skeleton $\pi^{a}$ violating a particular property, it is inherently \textit{state aware} and \textit{property driven}.}\syed{Need to revise the ``inherently state-aware part''} 
%
%To perform mutation on a selected transition $\mathcal{R}(q_c, \alpha, \gamma, q_n)$, \system performs two types of mutations described as follows.
%
For mutations, \system essentially performs two types of operations on a selected transition $\mathcal{R}$ as discussed below. 

%\syed{Please connect the following discussion with insight I3. The connection is loose in the current write-up. Our mutations are of two types and they have two goals: state-aware and property-driven.}
\noindent\ding{111} \textbf{M1: Mutating the observation of a transition.} 

\system{} alters the observation $(\alpha/\gamma)$ of $\mathcal{R}$,  i.e., alters either the input $\alpha$ or the output $\gamma$ or both based on the input and output in trace skeleton \tracesup{a} when the execution reaches at $q_c$. 

%The goal of this mutation kind is to either (i) mutate the input and output message of a transition at state $q_c$ to satisfy an input symbol in the given test skeleton $\pi^{a}$, or 
%(ii) mutate the input message to observe a deviation, i.e., a behavior in the target implementation \pimp different from what the guiding PSM suggests, such as acceptance of a prohibited message at a certain state.
%(ii) mutate the input message to observe a deviation, such as the target implementation \pimp accepting a prohibited message at a specific state, differing from what the guiding PSM suggests.

%
% The goal of this mutation kind is to either (i) mutate the input and output message of a transition at state $q_c$ to satisfy an input symbol in the given test skeleton $\pi^{a}$, or (ii) mutate the input message to observe any deviation, i.e., a behavior in the target implementation \pimp different from what the guiding PSM suggests, such as acceptance of a prohibited message at a certain state.
%
%Since we mutate the observation of a defined transition from the guiding FSM at a specific state, we ensure that only certain input messages, which are likely to be accepted by the target implementation at that state, are mutated. This contrasts with traditional fuzzers that randomly select messages to mutate without considering the device's current state.  
%
%We consider the first objective when we generate a concrete trace from a given trace skeleton $\pi^{a}$ (\S\ref{sec:tracebuilder:trace_generation}). 
%At a certain state $q_c$, suppose we require a specific input $\alpha'$ and output $\gamma'$ according to the given test skeleton, and it is not prescribed by the guiding PSM $\mathcal{M}$ at $q_c$. 

If the trace skeleton \tracesup{a} requires input $\alpha'$ and output $\gamma'$ at state $q_c$ but the guiding PSM $\mathcal{M}$ does not have $\alpha'/\gamma'$at $q_c$, to ensure the generated trace conforms with \tracesup{a}, we mutate the transition $\mathcal{R}$ in $\mathcal{M}$ with $\alpha'$ to obtain input $\alpha'$ and output $\gamma'$, i.e., $\mathcal{R}'(q_c, \alpha', \gamma', q_n)$. For example, in Figure 1, suppose at state $q_5$ if we require output \footnotesize\textsc{GUTI\_ reallocation \_complete}\normalsize\xspace for input
\footnotesize\textsc{GUTI\_ reallocation \_command: Replay ==1}\normalsize\xspace according to the test skeleton. However, since it is not prescribed at state $q_5$, we mutate the transition with observation $a_{gc}$ (with input \footnotesize\textsc{GUTI\_ reallocation \_command}\normalsize\xspace) to obtain input \footnotesize\textsc{GUTI\_ reallocation \_command: Replay == 1}\normalsize\xspace and output \footnotesize\textsc{GUTI\_ reallocation \_complete}\normalsize\xspace.
This mutation strategy is required to generate traces that satisfy a given test skeleton and test for violations of its associated security property.

\input{tables/mutation_operation}

%We consider the second objective when we are instantiating the wildcard characters of a test skeleton $\pi^{a}$, and decide to test with a mutated version of an input message to detect any deviation from the PSM that can lead to a security property violation. 

On the other hand, if \tracesup{a} has a wildcard character at state $q_c$, \system{} instantiates the wildcard character with a mutated version of an input message $\alpha$ to detect any deviation from the PSM that can lead to a security property violation. 
To increase the likelihood of a mutated message being accepted by a practical protocol implementation, \system{} considers the semantic meaning of the input message. It performs one of the six semantic operations. We summarize these operations with examples in Table \ref{tab:mutation_ops_m1}. These operations consider the semantics of the message fields, their defined values and ranges according to the protocol specification, and overall message semantics (e.g., plaintext or replayed version). As an example, in Figure \ref{fig:mutation_kind_example}(i), consider a mutation of the transition with observation $a_{ap}$ (with input \footnotesize\textsc{attach\_ accept: integrity == 0 \& cipher == 0 \& security\_ header \_ type == 0}\normalsize\xspace, marked blue) at state $q_1$. If we perform \textbf{OP2} operation and change the value of the \footnotesize\textsc{security\_ header \_ type}\normalsize\xspace  field to a prohibited value 4, we obtain the mutated message $a_{ap}'$ with input \footnotesize\textsc{attach\_ accept: integrity == 0 \& cipher == 0 \& security\_ header \_ type == 4}\normalsize\xspace. If the target implementation accepts this mutated message, we obtain a response (e.g., \footnotesize\textsc{attach\_ complete}\normalsize\xspace), which deviates from the guiding PSM.

% \updated{
% Furthermore, to incorporate mutations that have semantic meaning, we consider performing certain operations that alter the field value or a general property of the original message. To mutate any input message $\alpha$, we perform any of the six operators mentioned in Table \ref{tab:mutation_ops_m1}. After applying any of the operators, we obtain a mutated input message, and hence a mutated observation over a transition. 
% }

% \updated{
% For operation \textbf{OP1}, we select a particular message field and set it to a random value within its defined range according to the protocol specification. For example, in a \connectionreq message in BLE, we can set the 5-bit \textit{Hop} field to a value between 5 and 16. For operation \textbf{OP2}, we change the value of a particular field to a prohibited or reserved value. For instance, in a \connectionreq message in BLE, we can set the 5-bit \textit{Hop} field to a value greater than the maximum defined range of 16. This operation also includes setting incorrect key values in specific messages, such as sending a \keyexchange message in BLE with incorrect key values. For operation \textbf{OP3}, we set a field to its boundary values. For example, we can mutate a \connectionreq message by setting the \textit{channelMap} field to 0. For operation \textbf{OP4}, we send a plaintext version of a message that is typically expected to be integrity-protected and/or ciphered. For example, we can send an \attachacc message in 4G LTE in plaintext. For operation \textbf{OP5}, we combine multiple operations from \textbf{OP1} through \textbf{OP4}, allowing for the mutation of multiple fields simultaneously. This approach can be particularly useful for uncovering complex bugs. For example, we can send an \authreq message in 4G LTE with the separation bit set to 0 and the security header type set to 3. Finally, for operation \textbf{OP6}, we replay a previously captured instance of the message we are mutating. For example, we can send a replayed \smcmd message in 4G LTE after the NAS security context has been established. These mutation operations are designed to introduce meaningful variations in the input messages, with the goal of uncovering security vulnerabilities and unexpected deviations in protocol behavior.
% } 
%\syed{Incorporate the examples into the table in a new column.}
\begin{figure}[htbp]
\centering
% Begin first minipage for M1
\begin{minipage}{0.45\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tikzpicture}[>=stealth',bend angle=45,auto]

\tikzstyle{state}=[circle,thick,draw=black!100,fill=white!20,minimum size=1.2cm,text width=1.5cm,align=center,inner sep=0pt,line width=1mm]
\tikzstyle{edgeLabel}=[pos=0.5,text centered,text width=5cm,font={\sffamily\fontGuidingFSMFig}];  % Adjusted font size here
\tikzset{every loop/.style={min distance=1mm,looseness=3}}

\begin{scope}[->,node distance=4.2cm,yshift=0mm, xshift=-135mm, local bounding box=a_nodes]
% First net
\node [state, name=q0] {\fontGuidingFSMFig q0};
\node [state, name=q1, right of=q0, yshift=0mm] {\fontGuidingFSMFig q1};
\node [state, name=q2, right of=q1, yshift=0mm] {\fontGuidingFSMFig q2};
\node [state, name=q3, right of=q2, yshift=0mm] {\fontGuidingFSMFig q3};
\node [state, name=q4, right of=q3, yshift=0mm] {\fontGuidingFSMFig q4};
\node [state, name=q5, right of=q4, yshift=0mm] {\fontGuidingFSMFig q5};

\path[every node/.style={font=\sffamily\Large,inner sep=0pt}]
    (q0) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ea}$} (q1)
    (q1) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ar}$} (q2)

    % (q1) edge[red, loop above, out=120, in=60, looseness=5, yshift=20mm,  densely dashed, line width=1mm] node[edgeLabel, line width=1mm] {\fontGuidingFSMFig$a_{ac'}$} (q1)

    (q1) edge[blue, loop below, out=125, in=55, looseness=6, line width=1mm] node[edgeLabel, yshift=10mm, xshift=0mm] {\fontGuidingFSMFig$a_{ap}$} (q1)

    
    (q2) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{sm}$} (q3)
    (q3) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{rs}$} (q4)
    (q3) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=3mm, xshift=0mm, line width=1mm] {$a_{id}$} (q3)

    (q3) edge[bend right=-60, line width=1mm] node[edgeLabel,yshift=-2mm,xshift=2mm] {\fontGuidingFSMFig$a_{dr}$} (q0)
    (q5) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gc}$} (q5)
    (q5) edge[loop below, out=-120, in=-60, looseness=5, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gr}$} (q5)

    % new add for mutation - ridwan
    (q1) edge[red, loop below, out=-125, in=-55, looseness=6, densely dashed, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{ap'}$} (q1)

    % (q1) edge[red, bend right=-40, densely dashed, line width=1mm] node[edgeLabel,yshift=2mm,xshift=-8mm] {\fontGuidingFSMFig$a_{ac'}$} (q5)
    
    
    (q4) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ac}$} (q5);
\end{scope}
\end{tikzpicture}
}
\textbf{(i) Mutation Kind $\mathbf{M1}$}
\end{minipage}
% Begin second minipage for M2
\begin{minipage}{0.45\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tikzpicture}[>=stealth',bend angle=45,auto]
    
    \tikzstyle{state}=[circle,thick,draw=black!100,fill=white!20,minimum size=1.2cm,text width=1.5cm,align=center,inner sep=0pt,line width=1mm]
    \tikzstyle{edgeLabel}=[pos=0.5,text centered,text width=5cm,font={\sffamily\fontGuidingFSMFig}];  % Adjusted font size here
    \tikzset{every loop/.style={min distance=1mm,looseness=3}}
    
    \begin{scope}[->,node distance=4.2cm,yshift=0mm, xshift=-135mm, local bounding box=a_nodes]
    % First net
    \node [state, name=q0] {\fontGuidingFSMFig q0};
    \node [state, name=q1, right of=q0, yshift=0mm] {\fontGuidingFSMFig q1};
    \node [state, name=q2, right of=q1, yshift=0mm] {\fontGuidingFSMFig q2};
    \node [state, name=q3, right of=q2, yshift=0mm] {\fontGuidingFSMFig q3};
    \node [state, name=q4, right of=q3, yshift=0mm] {\fontGuidingFSMFig q4};
    \node [state, name=q5, right of=q4, yshift=0mm] {\fontGuidingFSMFig q5};
    
    \path[every node/.style={font=\sffamily\Large,inner sep=0pt}]
        (q0) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ea}$} (q1)
        (q1) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ar}$} (q2)
    
        % (q1) edge[red, loop above, out=120, in=60, looseness=5, yshift=20mm,  densely dashed, line width=1mm] node[edgeLabel, line width=1mm] {\fontGuidingFSMFig$a_{ac'}$} (q1)
    
        (q1) edge[blue, loop below, out=125, in=55, looseness=6,line width=1mm] node[edgeLabel, yshift=10mm, xshift=0mm] {\fontGuidingFSMFig$a_{ap}$} (q1)
    
        
        (q2) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{sm}$} (q3)
        (q3) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{rs}$} (q4)
        (q3) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=3mm, xshift=0mm, line width=1mm] {$a_{id}$} (q3)
    
        (q3) edge[bend right=-60, line width=1mm] node[edgeLabel,yshift=-3mm,xshift=-9mm] {\fontGuidingFSMFig$a_{dr}$} (q0)
        (q5) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gc}$} (q5)
        (q5) edge[loop below, out=-120, in=-60, looseness=5, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gr}$} (q5)
    
        % new add for mutation - ridwan
        % (q5) edge[red, loop below, out=-135, in=-45, looseness=10, densely dashed, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gr'}$} (q5)
    
        (q1) edge[red, bend right=-40, densely dashed, line width=1mm] node[edgeLabel,yshift=2mm,xshift=-8mm] {\fontGuidingFSMFig$a_{ap}$} (q5)
        
        
        (q4) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ac}$} (q5);
    \end{scope}
    \end{tikzpicture}
}
\textbf{(ii) Mutation Kind $\mathbf{M2}$}
\end{minipage}
\caption{Two types of Mutations M1 and M2. The transition labels are presented in Table \ref{tab:ble_running_example_table}.}
\label{fig:mutation_kind_example}
\end{figure}


\noindent\ding{111} \textbf{M2: Mutating the destination state of a transition.} 
%
In this case, we alter the destination state $q_n$ of a selected transition $\mathcal{R}$ $(q_c, \alpha, \gamma, q_n)$. The goal of this kind of mutation is to test whether the input message $\alpha$ at state $q_c$ leads to a state $q_m$ different than what is expected  by the guiding PSM (in this case $q_n$), which in turn can lead to an observable deviation or security property violation. This kind of mutation enables \system to detect certain bypass attacks (e.g., check whether any intermediate step can be bypassed to reach a secure state). 

% \system generates an instantiated trace that tests whether input message $\alpha$ at state $q_c$ leads to a state $q_m$ different than what is expected (in this case $q_n$) by the guiding PSM, which in turn can lead to an observable deviation or security property violation. This kind of mutation also enables \system to detect certain bypass attacks (e.g., check whether any intermediate step can be bypassed to reach a secure state). 

As an example, in Figure \ref{fig:mutation_kind_example}(ii), suppose we perform mutation over the transition with observation $a_{ac'}$ at state $q_1$ (marked blue). We can perform a mutation over the next state $q_2$ of the transition by changing the next state of the transition to $q_5$. This mutation would generate an instantiated trace that tests whether the target implementation incorrectly reaches state $q_5$ if a plaintext \attachacc is fed at state $q_1$.


\vspace{-0.3cm}
\subsection{Instantiated Trace Generation}\label{sec:tracebuilder:trace_generation}
%\textcolor{blue}{Finally, for a given trace skeleton \tracesup{a}, the challenge is to design an automatic approach to generate test traces $\gamma$ that would (1) satisfy the regular expression $\sigma_i$, (2) align with the guiding PSM $\mathcal{M}$, (3) ensure that each generated trace $\gamma$ require at most $\mu$ mutations on $\mathcal{M}$, and (4) maintain a maximum length of $\lambda$.} 

Given a test skeleton \tracesup{a} representing violation of a property $\phi \in \Phi$, a guiding PSM $\mathcal{M}$, a mutation budget $\mu$ and a length budget $\lambda$, we leverage insight \textbf{I2} and solve the problem of generating instantiated traces by combining the solutions of overlapping subproblems. For this, we formulate a dynamic programming problem as follows.

%textcolor{red}{originating from the destination state of a trace in $\mathcal{M}$ to a particular state in the trace.} \syed{Hard to understand} For this, we formulate a dynamic programming algorithm as follows.

% \begin{tcolorbox}
$\mathbf{\mathcal{G}(\mathcal{M}, \tracesup{a}, q_c, \mu, \lambda)}$: \emph{At any state $\mathsf{q}_c \in \mathcal{Q}$ of a guiding PSM $\mathcal{M}$, we want to craft a set of instantiated traces $\mathcal{T}$, where each instantiated trace (i) satisfies the test skeleton \tracesup{a}, (ii) is the outcome of a maximum of $\mu$ mutations applied on any trace in the guiding PSM $\mathcal{M}$ and (iii) is within a maximum length $\lambda$.}     
% \end{tcolorbox}

We use $\mathcal{G}(\mathcal{M}, \tracesup{a}, q_c, \mu, \lambda)$ to denote the problem which we can solve by leveraging the solution to its \emph{overlapping subproblems}. Consider we are at state $q_i$ of our guiding PSM $\mathcal{M}$ and we need to satisfy the $j^{th}$ observation $l_j$ = $(\alpha_j/\gamma_j)$ of the test skeleton \tracesup{a} (i.e, the test skeleton up to input symbol $l_{j-1}$ has been satisfied) and the next wildcard character in \tracesup{a} is $l_k$. Also, consider at $q_i$ the remaining mutation budget is $\mu_{i}$ and the remaining length budget is $\lambda_i$. For this problem, we consider the following four cases, where we formulate subproblems and prepend observations according to the following case.

\textbf{Case I.} If there is a transition $\mathcal{R}(q_i, \alpha, \gamma, q_m)$ at state $q_i$ whose observation satisfies $l_j$, \dpalgo can leverage solutions from the destination state $q_m$ that satisfies \tracesup{a} from observation $l_{j+1}$, with mutation budget $\mu_{i}$ and length budget $\lambda_i - 1$. \dpalgo prepends $l_j$ to the instantiated traces being generated from the subproblem. Since it places an observation ($l_j$) in the instantiated trace, it uses length budget $\lambda_i - 1$ to formulate the subproblem.

\textbf{Case II.} If there is no transition whose observation satisfies $l_j$, \dpalgo can consume a mutation to mutate the transition for $\alpha_j$ (the input message of observation $l_j$) to place observation $l_j$ in the instantiated trace, using mutation kind \textbf{M1}. Again \dpalgo leverages traces from the destination state of the transition $q_m$ that satisfies \tracesup{a} from observation $l_{j+1}$, with length budget $\lambda_i - 1$ but with mutation budget $\mu_i - 1$ since it consumed a mutation to place $l_j$. \dpalgo prepends $l_j$ to the obtained instantiated traces from the subproblem.

\textbf{Case III.} If there is a transition $\mathcal{R}(q_i, \alpha, \gamma, q_m)$ at state $q_i$ whose observation $(\alpha/\gamma)$ satisfies wildcard character element $l_k$, \dpalgo leverages solutions from the destination state $q_m$ that satisfies \tracesup{a} from observation $l_{j}$ with mutation budget $\mu_{i}$ and length budget $\lambda_i - 1$. It prepends observation $(\alpha/\gamma)$ to the obtained instantiated traces from the subproblem.

\textbf{Case IV.} Finally, for any transition $\mathcal{R}(q_i, \alpha, \gamma, q_m)$ at state $q_i$, \dpalgo can mutate the transition's observation and place a mutated observation $(\alpha/\gamma)_m$ using mutation kind \textbf{M1}. \dpalgo can leverage solutions from the destination state $q_m$ that satisfies \tracesup{a} from observation $l_{j}$ with length budget $\lambda_i - 1$ and also mutation budget $\mu_i - 1$ since we perform a mutation. It prepends the mutated observation $(\alpha/\gamma)_m$ to the obtained instantiated traces from the subproblem. Note that, we only place a \textit{mutation marker} in this case. This marker would be resolved by the \textit{mutation resolver} component of \dispatcher (\S\ref{sec:trace_dispatcher}) later on though operating on the input message $\alpha$ using one of the six operations described in \S\ref{sec:tracebuilder:mutation}. Note that, by placing various mutated message in place of the mutation marker, we can generate multiple traces to test OTA. 

Furthermore, for each case, \dpalgo may also consider mutating the destination state of the selected transition (mutation kind \textbf{M2}). In that case, \dpalgo mutates the destination state to another state $q_{mut}$ and formulates the subproblem from state $q_{mut}$ with mutation budget $\mu - 1$. \dpalgo will terminate if either \tracesup{a} is satisfied or it runs out of mutation or length budget.




%A detailed algorithm for \dpalgo is provided in Algorithm \ref{algo:tracebuilder} in Appendix and the base and recursive steps of the proposed dynamic programming algorithm are discussed in Appendix. 

%\syed{Need to discuss the cases of DP algorithm briefly here. For example, what happens if the j-th position of the RE is a literal/kleene star and that matches/doesn't match with the i-th symbol in a trace in M. When there is no match, the algorithm introduces mutations, i.e., mutation marker. The previous paragraph should be revised according to this suggestion. Also, when we say M in this algorithm, it is actually a trace in M in each iteration. If we can make this discussion simple, we do not need to introduce forward transition and allowed transition discussed in Appendix.} 


% Like any dynamic programming Algorithm, Tracebuilder also has a base case and a recursive step. \dpalgo considers mutations on the given guiding PSM \pimp to generate test traces. We first discuss the extraction of our guiding PSM. Then we discuss our notion of \textit{mutation} in detail. Finally we discuss the base case and recursive steps of \dpalgo.
%\input{algorithms/tracebuilder}





% For mutation kind \textbf{M1}, for each message type, we consider a \textit{mutation pool} which is a set of mutated variations of that message type (e.g. for \textsl{enc\_pause\_req} we consider \textsl{enc\_pause\_req: integrity == 0 \& replay == 0} and \textsl{enc\_pause\_req: integrity == 1 \& replay == 1} ). We consider a message from this mutation pool whenever a message needs to be mutated. Also, for mutation kind \textbf{M2}, for each state $q_c$, we consider the mutated next state $q_m$ among a given set of states. These sets and mutation pool can also be considered input to \system.

%  Proteus randomly applies one perturbation from a pool of available strategies. For example, it replaces an integrity protected message with a plaintext or a replayed one, or varies security sensitive fields (e.g., identity type in Identity Request, security header type etc.) in messages, and their combination thereof (e.g., plaintext identity request with identity type 3 (TMSI) and security header type 1).

% 



==> sections/7_tracebuilder_1_pm.tex <==
\section{\dpalgo: Generating Test Cases from Test Skeletons and Guiding PSM}
\label{sec:tracebuilder}
% Given a test skeleton \tracesup{a} representing violations of a security property $\phi \in \Phi$ and a guiding PSM $\mathcal{M}$, \system mutates $\mathcal{M}$ to efficiently generate meaningful test cases \tracesup{c} with the shape of \tracesup{a}. 
Given a test skeleton \tracesup{a} representing violations of a security property $\phi \in \Phi$, \system uses a guiding PSM $\mathcal{M}$ and mutates $\mathcal{M}$ to efficiently generate meaningful test cases \tracesup{c} with the shape of \tracesup{a}. 
%
{Note that the guiding PSM used by Proteus can be abstract compared to PSMs extracted from target device implementations. As a result, they are substantially smaller than PSMs learned from commercial devices (\S\ref{sec:experiments}). One can also use PSMs directly obtained from RFCs (e.g., \cite{rfc9293}) as a guiding FSM. Since \system does not require such detailed PSMs, it alleviates the manual effort required to obtain such PSMs or the prohibitively high time required to learn a detailed PSM from target implementations.} 
In what follows, 
we discuss our PSM mutation strategies, and  
% $\mathcal{M}$ 
% tailored for testing protocol implementations. We 
then present our test case generation mechanism.  %that takes into account the test skeleton(s), $\mathcal{M}$, mutation budget $\mu$ and length budget $l$ to construct effective traces. 


%construction technique to automatically we formulate a dynamic programming algorithm. Formally, the dynamic programming problem is formulated as follows.
\begin{comment}
\subsection{Constructing a Guiding PSM}
\todo{Modify}
% \ishtiaq{in my opinion, we need a subsection before this one that discusses alphabet and scope. based on that, we can write PSM construction. Without knowing the scope/alphabet, it is not possible to define/extract the PSM.}

%\system requires a guiding PSM as input to generate test traces. 
To construct a guiding PSM for a black-box protocol implementation, one can infer the PSM using black-box automata learning \cite{dikeue, blediff} \citereq through input/output observations or extract the PSM from the protocol specification. Since automata learning is prohibitively expensive and PSM construction is not the main focus of this paper, we leverage an existing natural language processing (NLP)-based technique, Hermes \cite{hermes}, to extract an PSM from protocol specifications. 

% \syed{Summarize the workflow of HERMES in one paragraph here.} \mukit{@Ishtiaq}
Hermes, at first, takes natural language specifications and 
uses a neural constituency parsing technique to identify transition components, e.g., conditions, actions, and states.
For instance, in the text, ``Upon receipt of the IDENTITY REQUEST message, the UE shall send an IDENTITY RESPONSE message to the network,'' Hermes marks ``Upon receipt \dots{} message'' as the condition and ``the UE shall \dots{} network'' as the action.
It then generates a logical formula for each component using a rule-based approach, leveraging a deep learning-based dependency parser and a domain-specific language. 
For the same example, ``the UE shall \dots{} network'' is translated to ``$\mathsf{channel\_ue\_to\_mme} = \mathsf{identity\_response}$.''
After that, these formulas for different transition components are then compiled into transitions.
Hermes then assembles all generated transitions, checks for inconsistencies, and finally constructs a finite state machine for the system. 

% It then translates each transition component to logical formulas and finally compiles them into an PSM. 
% As discussed in \todo{REF}, we first define our scope and alphabet.
% Then, according to the scope and the defined alphabet,
% we provide natural language specifications to Hermes to extract the PSMs. 
% Further, the Hermes-extracted PSM relies on many internal state variables as well as input messages to make transitions. 
% On the other hand, as a black box testing framework, \system needs an PSM with an observational form, i.e., transitions with input and output messages. 
% Thus, we leverage UEGEN from Hermes to convert the extracted PSM to the required observational form. 
% of PSM, which demonstrates the output of the device under test upon receiving different inputs in different states.
% \ishtiaq{please take a look if ``observational form'' makes sense.}

The PSMs generated by HERMES may contain some incorrect transitions, i.e., wrong source or destination state, or wrong conditions (i.e., inputs) or actions (outputs) of a transition.  
To tackle this, \system{}'s technique of incorporating test skeletons and mutations into test generation does not necessarily require an error-free guiding PSM for testing. However, the accuracy of the guiding PSM impacts its efficiency in detecting vulnerabilities, as we demonstrate through an experiment provided in Section \todo{\textbf{[REF]}}. 

%Additionally, \system requires an input and output alphabet consisting of message types and their associated predicates. Hermes not only provides a detailed PSM from the specifications but also provides a set of messages and predicates (e.g., different fields and their values). We construct the input and output alphabet of \system by utilizing the extracted set of messages and predicates from Hermes.
\end{comment}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/mutation_example_ccs_v1.pdf}
%     \caption{Example of Mutations on guiding PSM. The original PSM is shown in Figure \ref{fig:ble_running_example}. The red transitions are the mutated transitions.
%     }
%     \label{fig:mutation_example}
% \end{figure}

\begin{comment}
    \subsection{Mutating a PSM}
\label{sec:tracebuilder:mutation}
As discussed in challenge \textbf{C3} in \todo{Section~\ref{sec:design_challenges}}, since the guiding PSM is assumed to satisfy all security properties, we need to mutate the guiding PSM $\mathcal{M}$, i.e., PSM transitions to generate traces satisfying the regular expression \tracesup{a}, which signifies the violation of a security property. 
To perform mutation over a given transition $\mathcal{R}(q_c, \alpha, \beta, q_n)$, 
%where $q_c$ and $q_n$ are source and destination states, and $\alpha$ and $\beta$ are input and output of that transition, respectively, 
\system primarily performs two types of mutations:  (\textbf{M1}) mutation over the observation of a transition to trigger the input/output observation ${(\alpha, \beta)}_m$, and (\textbf{M2}) mutation over the destination state of a transition $q_n$, leading to a destination state $q_m \in \mathcal{Q} (q_m \neq q_n)$. 

Mutation type \textbf{M1} leads to the generation of traces where a mutated version of input message $\alpha$ is tested when the target implementation $\mathcal{I}_{P}$ reaches state $q_c$, with the hope of triggering a security property violation or a deviation (a behavior different from what the guiding PSM suggests). For this kind of mutation, \system randomly applies one perturbation from a %\textit{mutation pool}, which is 
a pool of mutation strategies. For example, it replaces an integrity-protected message with a plaintext or a replayed one, or varies security-sensitive fields (e.g., in LTE, security header type, identity type in identity request message) in messages, and their combination thereof (e.g., plaintext identity request with identity type 3 (TMSI) and security header type 1).


Mutation type \textbf{M2} generates a trace that tests whether input message $\alpha$ at state $q_c$ leads to a state $q_m$ different than what is expected (in this case $q_n$) by the guiding PSM, which in turn can lead to an observable deviation or security property violation. This kind of mutation also enables \system to detect certain bypass attacks. For example, the logical flow of SC (Secure Connections) key pairing in BLE is \keyexchange, \smrandomsend, \dhkeycheck, \encreq. More specifically, if \system considers mutating the destination state of the key exchange message to the state for \dhkeycheck, \system can test whether bypassing \smrandomsend is possible.


As examples of mutation kinds \textbf{M1} and \textbf{M2}, consider the examples shown in Figure \ref{fig:mutation_example}. Suppose we are performing mutation over the transition $\mathcal{R}$($q_4$,\encpausereqbenignfull, \nullaction, $q_4$). As an example of mutation kind \textbf{M1}, we can perform mutation over the observation $a_{ep}$, and and test it with mutated observation ${(a_{ep})}_m$. A practical example of mutation over $a_{ep}$ could be testing with input \encpausereqreplay, which tests whether the target implementation properly handles the message at state $q_4$ or not. As an example of mutation kind \textbf{M2}, we can perform a mutation over the next state $q_4$ of the transition by changing the next state of the transition to $q_0$. This mutation would generate a trace that tests whether the target implementation incorrectly goes back to state $q_0$ if \encpausereqbenignfull is fed at state $q_4$.
\end{comment}

%\vspace{-2mm}
\subsection{Mutating a PSM}
\label{sec:tracebuilder:mutation}

As discussed in challenge \textbf{C2} in \S\ref{sec:overview_and_challenges}, since the guiding PSM is assumed to satisfy all security properties, we need to mutate the guiding PSM $\mathcal{M}$, i.e., PSM transitions to generate traces satisfying a test skeleton \tracesup{a}, which signifies the violation of a security property. \system selects a transition $\mathcal{R}(q_c, \alpha, \gamma, q_n)$ to mutate while generating concrete traces satisfying a test skeleton \tracesup{a} as described in detail in \S\ref{sec:tracebuilder:trace_generation}. 
%\textcolor{red}{Since this selection is based on the defined transitions in the guiding PSM and driven by the goal of satisfying a test skeleton $\pi^{a}$ violating a particular property, it is inherently \textit{state aware} and \textit{property driven}.}\syed{Need to revise the ``inherently state-aware part''} 
%
%To perform mutation on a selected transition $\mathcal{R}(q_c, \alpha, \gamma, q_n)$, \system performs two types of mutations described as follows.
%
For mutations, \system essentially performs two types of operations on a selected transition $\mathcal{R}$ as discussed below. 

%\syed{Please connect the following discussion with insight I3. The connection is loose in the current write-up. Our mutations are of two types and they have two goals: state-aware and property-driven.}
\noindent\ding{111} \textbf{Mutation kind M1: Mutating the observation of a transition.} 
\system{} alters the observation $(\alpha/\gamma)$ of $\mathcal{R}$,  i.e., alters either the input $\alpha$ or the output $\gamma$ or both based on the input and output in trace skeleton \tracesup{a} when the execution reaches at $q_c$. 

%The goal of this mutation kind is to either (i) mutate the input and output message of a transition at state $q_c$ to satisfy an input symbol in the given test skeleton $\pi^{a}$, or 
%(ii) mutate the input message to observe a deviation, i.e., a behavior in the target implementation \pimp different from what the guiding PSM suggests, such as acceptance of a prohibited message at a certain state.
%(ii) mutate the input message to observe a deviation, such as the target implementation \pimp accepting a prohibited message at a specific state, differing from what the guiding PSM suggests.

%
% The goal of this mutation kind is to either (i) mutate the input and output message of a transition at state $q_c$ to satisfy an input symbol in the given test skeleton $\pi^{a}$, or (ii) mutate the input message to observe any deviation, i.e., a behavior in the target implementation \pimp different from what the guiding PSM suggests, such as acceptance of a prohibited message at a certain state.
%
%Since we mutate the observation of a defined transition from the guiding FSM at a specific state, we ensure that only certain input messages, which are likely to be accepted by the target implementation at that state, are mutated. This contrasts with traditional fuzzers that randomly select messages to mutate without considering the device's current state.  
%
%We consider the first objective when we generate a concrete trace from a given trace skeleton $\pi^{a}$ (\S\ref{sec:tracebuilder:trace_generation}). 
%At a certain state $q_c$, suppose we require a specific input $\alpha'$ and output $\gamma'$ according to the given test skeleton, and it is not prescribed by the guiding PSM $\mathcal{M}$ at $q_c$. 

If the trace skeleton \tracesup{a} requires input $\alpha'$ and output $\gamma'$ at state $q_c$ but the guiding PSM $\mathcal{M}$ does not have $\alpha'/\gamma'$at $q_c$, to ensure the generated trace conforms with \tracesup{a}, we mutate the transition $\mathcal{R}$ in $\mathcal{M}$ with $\alpha'$ to obtain input $\alpha'$ and output $\gamma'$, i.e., $\mathcal{R}'(q_c, \alpha', \gamma', q_n)$. For example, in Figure 1, suppose at state $q_5$ if we require output \footnotesize\textsc{GUTI\_ reallocation \_complete}\normalsize\xspace for input
\footnotesize\textsc{GUTI\_ reallocation \_command: Replay ==1}\normalsize\xspace according to the test skeleton. However, since it is not prescribed at state $q_5$, we mutate the transition with observation $a_{gc}$ (with input \footnotesize\textsc{GUTI\_ reallocation \_command}\normalsize\xspace) to obtain input \footnotesize\textsc{GUTI\_ reallocation \_command: Replay == 1}\normalsize\xspace and output \footnotesize\textsc{GUTI\_ reallocation \_complete}\normalsize\xspace.
This mutation strategy is required to generate traces that satisfy a given test skeleton and test for violations of its associated security property.

\input{tables/mutation_operation}

%We consider the second objective when we are instantiating the wildcard characters of a test skeleton $\pi^{a}$, and decide to test with a mutated version of an input message to detect any deviation from the PSM that can lead to a security property violation. 

On the other hand, if \tracesup{a} has a wildcard character at state $q_c$, \system{} instantiates the wildcard character with a mutated version of an input message $\alpha$ to detect any deviation from the PSM that can lead to a security property violation. 
To increase the likelihood of a mutated message being accepted by a practical protocol implementation, \system{} considers the semantic meaning of the input message. It performs one of the six semantic operations. We summarize these operations with examples in Table \ref{tab:mutation_ops_m1}. These operations consider the semantics of the message fields, their defined values and ranges according to the protocol specification, and overall message semantics (e.g., plaintext or replayed version). As an example, in Figure \ref{fig:mutation_kind_example}(i), consider a mutation of the transition with observation $a_{ap}$ (with input \footnotesize\textsc{attach\_ accept: integrity == 0 \& cipher == 0 \& security\_ header \_ type == 0}\normalsize\xspace, marked blue) at state $q_1$. If we perform \textbf{OP2} operation and change the value of the \footnotesize\textsc{security\_ header \_ type}\normalsize\xspace  field to a prohibited value 4, we obtain the mutated message $a_{ap}'$ with input \footnotesize\textsc{attach\_ accept: integrity == 0 \& cipher == 0 \& security\_ header \_ type == 4}\normalsize\xspace. If the target implementation accepts this mutated message, we obtain a response (e.g., \footnotesize\textsc{attach\_ complete}\normalsize\xspace), which deviates from the guiding PSM.
\vspace{-0.2cm}
% \updated{
% Furthermore, to incorporate mutations that have semantic meaning, we consider performing certain operations that alter the field value or a general property of the original message. To mutate any input message $\alpha$, we perform any of the six operators mentioned in Table \ref{tab:mutation_ops_m1}. After applying any of the operators, we obtain a mutated input message, and hence a mutated observation over a transition. 
% }

% \updated{
% For operation \textbf{OP1}, we select a particular message field and set it to a random value within its defined range according to the protocol specification. For example, in a \connectionreq message in BLE, we can set the 5-bit \textit{Hop} field to a value between 5 and 16. For operation \textbf{OP2}, we change the value of a particular field to a prohibited or reserved value. For instance, in a \connectionreq message in BLE, we can set the 5-bit \textit{Hop} field to a value greater than the maximum defined range of 16. This operation also includes setting incorrect key values in specific messages, such as sending a \keyexchange message in BLE with incorrect key values. For operation \textbf{OP3}, we set a field to its boundary values. For example, we can mutate a \connectionreq message by setting the \textit{channelMap} field to 0. For operation \textbf{OP4}, we send a plaintext version of a message that is typically expected to be integrity-protected and/or ciphered. For example, we can send an \attachacc message in 4G LTE in plaintext. For operation \textbf{OP5}, we combine multiple operations from \textbf{OP1} through \textbf{OP4}, allowing for the mutation of multiple fields simultaneously. This approach can be particularly useful for uncovering complex bugs. For example, we can send an \authreq message in 4G LTE with the separation bit set to 0 and the security header type set to 3. Finally, for operation \textbf{OP6}, we replay a previously captured instance of the message we are mutating. For example, we can send a replayed \smcmd message in 4G LTE after the NAS security context has been established. These mutation operations are designed to introduce meaningful variations in the input messages, with the goal of uncovering security vulnerabilities and unexpected deviations in protocol behavior.
% } 
%\syed{Incorporate the examples into the table in a new column.}

\begin{figure}[htbp]
\centering
% Begin first minipage for M1
\begin{minipage}{0.49\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tikzpicture}[>=stealth',bend angle=45,auto]

\tikzstyle{state}=[circle,thick,draw=black!100,fill=white!20,minimum size=2cm,text width=2cm,align=center,inner sep=0pt,line width=1mm]
\tikzstyle{edgeLabel}=[pos=0.5,text centered,text width=5cm,font={\sffamily\fontGuidingFSMFig}];  % Adjusted font size here
\tikzset{every loop/.style={min distance=1mm,looseness=3}}

\begin{scope}[->,node distance=4.2cm,yshift=0mm, xshift=-135mm, local bounding box=a_nodes]
% First net
\node [state, name=q0] {\fontGuidingFSMFig q0};
\node [state, name=q1, right of=q0, yshift=0mm] {\fontGuidingFSMFig q1};
\node [state, name=q2, right of=q1, yshift=0mm] {\fontGuidingFSMFig q2};
\node [state, name=q3, right of=q2, yshift=0mm] {\fontGuidingFSMFig q3};
\node [state, name=q4, right of=q3, yshift=0mm] {\fontGuidingFSMFig q4};
\node [state, name=q5, right of=q4, yshift=0mm] {\fontGuidingFSMFig q5};

\path[every node/.style={font=\sffamily\Large,inner sep=0pt}]
    (q0) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ea}$} (q1)
    (q1) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ar}$} (q2)

    % (q1) edge[red, loop above, out=120, in=60, looseness=5, yshift=20mm,  densely dashed, line width=1mm] node[edgeLabel, line width=1mm] {\fontGuidingFSMFig$a_{ac'}$} (q1)

    (q1) edge[blue, loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=3mm, xshift=0mm] {\fontGuidingFSMFig$a_{ap}$} (q1)

    
    (q2) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{sm}$} (q3)
    (q3) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{rs}$} (q4)
    (q3) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=3mm, xshift=0mm, line width=1mm] {$a_{id}$} (q3)

    (q3) edge[bend right=-65, line width=1mm] node[edgeLabel,yshift=-8mm,xshift=2mm] {\fontGuidingFSMFig$a_{dr}$} (q0)
    (q5) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gc}$} (q5)
    (q5) edge[loop below, out=-120, in=-60, looseness=5, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gr}$} (q5)

    % new add for mutation - ridwan
    (q1) edge[red, loop below, out=-115, in=-55, looseness=5, densely dashed, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{ap'}$} (q1)

    % (q1) edge[red, bend right=-40, densely dashed, line width=1mm] node[edgeLabel,yshift=2mm,xshift=-8mm] {\fontGuidingFSMFig$a_{ac'}$} (q5)
    
    
    (q4) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ac}$} (q5);
\end{scope}
\end{tikzpicture}
}
\textbf{(i) Mutation kind $\mathbf{M1}$}
\end{minipage}
% Begin second minipage for M2
\begin{minipage}{0.49\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tikzpicture}[>=stealth',bend angle=45,auto]
    
    \tikzstyle{state}=[circle,thick,draw=black!100,fill=white!20,minimum size=2cm,text width=2cm,align=center,inner sep=0pt,line width=1mm]
    \tikzstyle{edgeLabel}=[pos=0.5,text centered,text width=5cm,font={\sffamily\fontGuidingFSMFig}];  % Adjusted font size here
    \tikzset{every loop/.style={min distance=1mm,looseness=3}}
    
    \begin{scope}[->,node distance=4.2cm,yshift=0mm, xshift=-135mm, local bounding box=a_nodes]
    % First net
    \node [state, name=q0] {\fontGuidingFSMFig q0};
    \node [state, name=q1, right of=q0, yshift=0mm] {\fontGuidingFSMFig q1};
    \node [state, name=q2, right of=q1, yshift=0mm] {\fontGuidingFSMFig q2};
    \node [state, name=q3, right of=q2, yshift=0mm] {\fontGuidingFSMFig q3};
    \node [state, name=q4, right of=q3, yshift=0mm] {\fontGuidingFSMFig q4};
    \node [state, name=q5, right of=q4, yshift=0mm] {\fontGuidingFSMFig q5};
    
    \path[every node/.style={font=\sffamily\Large,inner sep=0pt}]
        (q0) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ea}$} (q1)
        (q1) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ar}$} (q2)
    
        % (q1) edge[red, loop above, out=120, in=60, looseness=5, yshift=20mm,  densely dashed, line width=1mm] node[edgeLabel, line width=1mm] {\fontGuidingFSMFig$a_{ac'}$} (q1)
    
        (q1) edge[blue, loop above, out=120, in=60, looseness=5,line width=1mm] node[edgeLabel, yshift=3mm, xshift=0mm] {\fontGuidingFSMFig$a_{ap}$} (q1)
    
        
        (q2) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{sm}$} (q3)
        (q3) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{rs}$} (q4)
        (q3) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=3mm, xshift=0mm, line width=1mm] {$a_{id}$} (q3)
    
        (q3) edge[bend right=-60, line width=1mm] node[edgeLabel,yshift=-3mm,xshift=-9mm] {\fontGuidingFSMFig$a_{dr}$} (q0)
        (q5) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gc}$} (q5)
        (q5) edge[loop below, out=-120, in=-60, looseness=5, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gr}$} (q5)
    
        % new add for mutation - ridwan
        % (q5) edge[red, loop below, out=-135, in=-45, looseness=10, densely dashed, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gr'}$} (q5)
    
        (q1) edge[red, bend right=-50, densely dashed, line width=1mm] node[edgeLabel,yshift=2mm,xshift=-8mm] {\fontGuidingFSMFig$a_{ap}$} (q5)
        
        
        (q4) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ac}$} (q5);
    \end{scope}
    \end{tikzpicture}
}
\textbf{(ii) Mutation kind $\mathbf{M2}$}
\end{minipage}
\caption{Two kinds of mutations M1 and M2. The transition labels are presented in Table \ref{tab:ble_running_example_table}.}
\label{fig:mutation_kind_example}
\end{figure}
\vspace{-0.3cm}

\noindent\ding{111} \textbf{Mutation kind M2: Mutating the destination state of a transition.} 
%
In this case, we alter the destination state $q_n$ of a selected transition $\mathcal{R}$ $(q_c, \alpha, \gamma, q_n)$. The goal of this kind of mutation is to test whether the input message $\alpha$ at state $q_c$ leads to a state $q_m$ different than what is expected  by the guiding PSM (in this case $q_n$), which in turn can lead to an observable deviation or security property violation. This kind of mutation enables \system to identify certain bypass attacks, e.g., detect whether any intermediate step can be bypassed to reach a secure state. 

% \system generates an instantiated trace that tests whether input message $\alpha$ at state $q_c$ leads to a state $q_m$ different than what is expected (in this case $q_n$) by the guiding PSM, which in turn can lead to an observable deviation or security property violation. This kind of mutation also enables \system to detect certain bypass attacks (e.g., check whether any intermediate step can be bypassed to reach a secure state). 

To illustrate, in Figure \ref{fig:mutation_kind_example}(ii), suppose we perform mutation over the transition with observation $a_{ac'}$ at state $q_1$ (marked blue). We can perform a mutation over the next state $q_2$ of the transition by changing the next state of the transition to $q_5$. This mutation would generate an instantiated trace that tests whether the target incorrectly reaches state $q_5$ if a plaintext \attachacc is fed at $q_1$.




%\vspace{-0.3cm}
\subsection{Instantiated Trace Generation}\label{sec:tracebuilder:trace_generation}
%\textcolor{blue}{Finally, for a given trace skeleton \tracesup{a}, the challenge is to design an automatic approach to generate test traces $\gamma$ that would (1) satisfy the regular expression $\sigma_i$, (2) align with the guiding PSM $\mathcal{M}$, (3) ensure that each generated trace $\gamma$ require at most $\mu$ mutations on $\mathcal{M}$, and (4) maintain a maximum length of $\lambda$.} 

Given a test skeleton \tracesup{a} representing violation of a property $\phi \in \Phi$, a guiding PSM $\mathcal{M}$, a mutation budget $\mu$ and a length budget $\lambda$, we leverage insight \textbf{I2} and solve the problem of generating instantiated traces by combining the solutions of overlapping subproblems. For this, we formulate a dynamic programming problem as follows.

%textcolor{red}{originating from the destination state of a trace in $\mathcal{M}$ to a particular state in the trace.} \syed{Hard to understand} For this, we formulate a dynamic programming algorithm as follows.

% \begin{tcolorbox}
$\mathbf{\mathcal{G}(\mathcal{M}, \tracesup{a}, q_c, \mu, \lambda)}$: \emph{At any state $\mathsf{q}_c \in \mathcal{Q}$ of a guiding PSM $\mathcal{M}$, we want to craft a set of instantiated traces $\mathcal{T}$, where each instantiated trace (i) satisfies the test skeleton \tracesup{a}, (ii) is the outcome of a maximum of $\mu$ mutations applied on any trace in the guiding PSM $\mathcal{M}$ and (iii) is within a maximum length $\lambda$.}     
% \end{tcolorbox}

We use $\mathcal{G}(\mathcal{M}, \tracesup{a}, q_c, \mu, \lambda)$ to denote the problem which we can solve by leveraging the solution to its \emph{overlapping subproblems}. Consider we are at state $q_i$ of our guiding PSM $\mathcal{M}$ and we need to satisfy the $j^{th}$ observation $l_j$ = $(\alpha_j/\gamma_j)$ of the test skeleton \tracesup{a} (i.e, the test skeleton up to input symbol $l_{j-1}$ has been satisfied) and the next wildcard character in \tracesup{a} is $l_k$. Also, consider at $q_i$ the remaining mutation budget is $\mu_{i}$ and the remaining length budget is $\lambda_i$. For this problem, we consider the following four cases, where we formulate subproblems and prepend observations according to the following case.

\textbf{Case I.} If there is a transition $\mathcal{R}(q_i, \alpha, \gamma, q_m)$ at state $q_i$ whose observation satisfies $l_j$, \dpalgo can leverage solutions from the destination state $q_m$ that satisfies \tracesup{a} from observation $l_{j+1}$, with mutation budget $\mu_{i}$ and length budget $\lambda_i - 1$. \dpalgo prepends $l_j$ to the instantiated traces being generated from the subproblem. Since it places an observation ($l_j$) in the instantiated trace, it uses length budget $\lambda_i - 1$ to formulate the subproblem.

\textbf{Case II.} If there is no transition whose observation satisfies $l_j$, \dpalgo can consume a mutation to mutate the transition for $\alpha_j$ (the input message of observation $l_j$) to place observation $l_j$ in the instantiated trace, using mutation kind \textbf{M1}. Again \dpalgo leverages traces from the destination state of the transition $q_m$ that satisfies \tracesup{a} from observation $l_{j+1}$, with length budget $\lambda_i - 1$ but with mutation budget $\mu_i - 1$ since it consumed a mutation to place $l_j$. \dpalgo prepends $l_j$ to the obtained instantiated traces from the subproblem.

\textbf{Case III.} If there is a transition $\mathcal{R}(q_i, \alpha, \gamma, q_m)$ at state $q_i$ whose observation $(\alpha/\gamma)$ satisfies wildcard character element $l_k$, \dpalgo leverages solutions from the destination state $q_m$ that satisfies \tracesup{a} from observation $l_{j}$ with mutation budget $\mu_{i}$ and length budget $\lambda_i - 1$. It prepends observation $(\alpha/\gamma)$ to the obtained instantiated traces from the subproblem.

\textbf{Case IV.} Finally, for any transition $\mathcal{R}(q_i, \alpha, \gamma, q_m)$ at state $q_i$, \dpalgo can mutate the transition's observation and place a mutated observation $(\alpha/\gamma)_m$ using mutation kind \textbf{M1}. \dpalgo can leverage solutions from the destination state $q_m$ that satisfies \tracesup{a} from observation $l_{j}$ with length budget $\lambda_i - 1$ and also mutation budget $\mu_i - 1$ since we perform a mutation. It prepends the mutated observation $(\alpha/\gamma)_m$ to the obtained instantiated traces from the subproblem. Note that, we only place a \textit{mutation marker} in this case. This marker would be resolved by the \textit{mutation resolver} component of \dispatcher (\S\ref{sec:trace_dispatcher}) later on though operating on the input message $\alpha$ using one of the six operations described in \S\ref{sec:tracebuilder:mutation}. Note that, by placing various mutated message in place of the mutation marker, we can generate multiple traces to test OTA. 

Furthermore, for each case, \dpalgo may also consider mutating the destination state of the selected transition (mutation kind \textbf{M2}). In that case, \dpalgo mutates the destination state to another state $q_{mut}$ and formulates the subproblem from state $q_{mut}$ with mutation budget $\mu - 1$. \dpalgo will terminate if either \tracesup{a} is satisfied or it runs out of mutation or length budget.




%A detailed algorithm for \dpalgo is provided in Algorithm \ref{algo:tracebuilder} in Appendix and the base and recursive steps of the proposed dynamic programming algorithm are discussed in Appendix. 

%\syed{Need to discuss the cases of DP algorithm briefly here. For example, what happens if the j-th position of the RE is a literal/kleene star and that matches/doesn't match with the i-th symbol in a trace in M. When there is no match, the algorithm introduces mutations, i.e., mutation marker. The previous paragraph should be revised according to this suggestion. Also, when we say M in this algorithm, it is actually a trace in M in each iteration. If we can make this discussion simple, we do not need to introduce forward transition and allowed transition discussed in Appendix.} 


% Like any dynamic programming Algorithm, Tracebuilder also has a base case and a recursive step. \dpalgo considers mutations on the given guiding PSM \pimp to generate test traces. We first discuss the extraction of our guiding PSM. Then we discuss our notion of \textit{mutation} in detail. Finally we discuss the base case and recursive steps of \dpalgo.
%\input{algorithms/tracebuilder}





% For mutation kind \textbf{M1}, for each message type, we consider a \textit{mutation pool} which is a set of mutated variations of that message type (e.g. for \textsl{enc\_pause\_req} we consider \textsl{enc\_pause\_req: integrity == 0 \& replay == 0} and \textsl{enc\_pause\_req: integrity == 1 \& replay == 1} ). We consider a message from this mutation pool whenever a message needs to be mutated. Also, for mutation kind \textbf{M2}, for each state $q_c$, we consider the mutated next state $q_m$ among a given set of states. These sets and mutation pool can also be considered input to \system.

%  Proteus randomly applies one perturbation from a pool of available strategies. For example, it replaces an integrity protected message with a plaintext or a replayed one, or varies security sensitive fields (e.g., identity type in Identity Request, security header type etc.) in messages, and their combination thereof (e.g., plaintext identity request with identity type 3 (TMSI) and security header type 1).

% 



==> sections/7_tracebuilder_backup.tex <==
\section{\dpalgo: Generating Test Cases from Test Skeletons and Guiding PSM}
\label{sec:tracebuilder}
Given a test skeleton \tracesup{a} representing violations of a security property $\phi \in \Phi$ and a guiding PSM $\mathcal{M}$, \system mutates $\mathcal{M}$ 
%, a mutation budget $\mu$ and a length budget $\lambda$, 
to efficiently generate meaningful test cases \tracesup{c} with the shape of \tracesup{a}. We now discuss 
%how we use an existing technique to automatically extract PSM from protocol specifications. We then illustrate 
our PSM mutation strategies, and  
% $\mathcal{M}$ 
% tailored for testing protocol implementations. We 
then present our test case generation mechanism.  %that takes into account the test skeleton(s), $\mathcal{M}$, mutation budget $\mu$ and length budget $l$ to construct effective traces. 


%construction technique to automatically we formulate a dynamic programming algorithm. Formally, the dynamic programming problem is formulated as follows.
\begin{comment}
\subsection{Constructing a Guiding PSM}
\todo{Modify}
% \ishtiaq{in my opinion, we need a subsection before this one that discusses alphabet and scope. based on that, we can write PSM construction. Without knowing the scope/alphabet, it is not possible to define/extract the PSM.}

%\system requires a guiding PSM as input to generate test traces. 
To construct a guiding PSM for a black-box protocol implementation, one can infer the PSM using black-box automata learning \cite{dikeue, blediff} \citereq through input/output observations or extract the PSM from the protocol specification. Since automata learning is prohibitively expensive and PSM construction is not the main focus of this paper, we leverage an existing natural language processing (NLP)-based technique, Hermes \cite{hermes}, to extract an PSM from protocol specifications. 

% \syed{Summarize the workflow of HERMES in one paragraph here.} \mukit{@Ishtiaq}
Hermes, at first, takes natural language specifications and 
uses a neural constituency parsing technique to identify transition components, e.g., conditions, actions, and states.
For instance, in the text, ``Upon receipt of the IDENTITY REQUEST message, the UE shall send an IDENTITY RESPONSE message to the network,'' Hermes marks ``Upon receipt \dots{} message'' as the condition and ``the UE shall \dots{} network'' as the action.
It then generates a logical formula for each component using a rule-based approach, leveraging a deep learning-based dependency parser and a domain-specific language. 
For the same example, ``the UE shall \dots{} network'' is translated to ``$\mathsf{channel\_ue\_to\_mme} = \mathsf{identity\_response}$.''
After that, these formulas for different transition components are then compiled into transitions.
Hermes then assembles all generated transitions, checks for inconsistencies, and finally constructs a finite state machine for the system. 

% It then translates each transition component to logical formulas and finally compiles them into an PSM. 
% As discussed in \todo{REF}, we first define our scope and alphabet.
% Then, according to the scope and the defined alphabet,
% we provide natural language specifications to Hermes to extract the PSMs. 
% Further, the Hermes-extracted PSM relies on many internal state variables as well as input messages to make transitions. 
% On the other hand, as a black box testing framework, \system needs an PSM with an observational form, i.e., transitions with input and output messages. 
% Thus, we leverage UEGEN from Hermes to convert the extracted PSM to the required observational form. 
% of PSM, which demonstrates the output of the device under test upon receiving different inputs in different states.
% \ishtiaq{please take a look if ``observational form'' makes sense.}

The PSMs generated by HERMES may contain some incorrect transitions, i.e., wrong source or destination state, or wrong conditions (i.e., inputs) or actions (outputs) of a transition.  
To tackle this, \system{}'s technique of incorporating test skeletons and mutations into test generation does not necessarily require an error-free guiding PSM for testing. However, the accuracy of the guiding PSM impacts its efficiency in detecting vulnerabilities, as we demonstrate through an experiment provided in Section \todo{\textbf{[REF]}}. 

%Additionally, \system requires an input and output alphabet consisting of message types and their associated predicates. Hermes not only provides a detailed PSM from the specifications but also provides a set of messages and predicates (e.g., different fields and their values). We construct the input and output alphabet of \system by utilizing the extracted set of messages and predicates from Hermes.
\end{comment}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/mutation_example_ccs_v1.pdf}
%     \caption{Example of Mutations on guiding PSM. The original PSM is shown in Figure \ref{fig:ble_running_example}. The red transitions are the mutated transitions.
%     }
%     \label{fig:mutation_example}
% \end{figure}

\begin{comment}
    \subsection{Mutating a PSM}
\label{sec:tracebuilder:mutation}
As discussed in challenge \textbf{C3} in \todo{Section~\ref{sec:design_challenges}}, since the guiding PSM is assumed to satisfy all security properties, we need to mutate the guiding PSM $\mathcal{M}$, i.e., PSM transitions to generate traces satisfying the regular expression \tracesup{a}, which signifies the violation of a security property. 
To perform mutation over a given transition $\mathcal{R}(q_c, \alpha, \beta, q_n)$, 
%where $q_c$ and $q_n$ are source and destination states, and $\alpha$ and $\beta$ are input and output of that transition, respectively, 
\system primarily performs two types of mutations:  (\textbf{M1}) mutation over the observation of a transition to trigger the input/output observation ${(\alpha, \beta)}_m$, and (\textbf{M2}) mutation over the destination state of a transition $q_n$, leading to a destination state $q_m \in \mathcal{Q} (q_m \neq q_n)$. 

Mutation type \textbf{M1} leads to the generation of traces where a mutated version of input message $\alpha$ is tested when the target implementation $\mathcal{I}_{P}$ reaches state $q_c$, with the hope of triggering a security property violation or a deviation (a behavior different from what the guiding PSM suggests). For this kind of mutation, \system randomly applies one perturbation from a %\textit{mutation pool}, which is 
a pool of mutation strategies. For example, it replaces an integrity-protected message with a plaintext or a replayed one, or varies security-sensitive fields (e.g., in LTE, security header type, identity type in identity request message) in messages, and their combination thereof (e.g., plaintext identity request with identity type 3 (TMSI) and security header type 1).


Mutation type \textbf{M2} generates a trace that tests whether input message $\alpha$ at state $q_c$ leads to a state $q_m$ different than what is expected (in this case $q_n$) by the guiding PSM, which in turn can lead to an observable deviation or security property violation. This kind of mutation also enables \system to detect certain bypass attacks. For example, the logical flow of SC (Secure Connections) key pairing in BLE is \keyexchange, \smrandomsend, \dhkeycheck, \encreq. More specifically, if \system considers mutating the destination state of the key exchange message to the state for \dhkeycheck, \system can test whether bypassing \smrandomsend is possible.


As examples of mutation kinds \textbf{M1} and \textbf{M2}, consider the examples shown in Figure \ref{fig:mutation_example}. Suppose we are performing mutation over the transition $\mathcal{R}$($q_4$,\encpausereqbenignfull, \nullaction, $q_4$). As an example of mutation kind \textbf{M1}, we can perform mutation over the observation $a_{ep}$, and and test it with mutated observation ${(a_{ep})}_m$. A practical example of mutation over $a_{ep}$ could be testing with input \encpausereqreplay, which tests whether the target implementation properly handles the message at state $q_4$ or not. As an example of mutation kind \textbf{M2}, we can perform a mutation over the next state $q_4$ of the transition by changing the next state of the transition to $q_0$. This mutation would generate a trace that tests whether the target implementation incorrectly goes back to state $q_0$ if \encpausereqbenignfull is fed at state $q_4$.
\end{comment}

%\vspace{-2mm}
\subsection{Mutating a PSM}
\label{sec:tracebuilder:mutation}

As discussed in challenge \textbf{C2} in section~\ref{sec:overview_and_challenges}, since the guiding PSM is assumed to satisfy all security properties, we need to mutate the guiding PSM $\mathcal{M}$, i.e., PSM transitions to generate traces satisfying a test skeleton \tracesup{a}, which signifies the violation of a security property. \system selects a transition $\mathcal{R}(q_c, \alpha, \gamma, q_n)$ to mutate while generating concrete traces satisfying a test skeleton \tracesup{a} as described in detail in \S\ref{sec:tracebuilder:trace_generation}. 
%\textcolor{red}{Since this selection is based on the defined transitions in the guiding PSM and driven by the goal of satisfying a test skeleton $\pi^{a}$ violating a particular property, it is inherently \textit{state aware} and \textit{property driven}.}\syed{Need to revise the ``inherently state-aware part''} 
%
%To perform mutation on a selected transition $\mathcal{R}(q_c, \alpha, \gamma, q_n)$, \system performs two types of mutations described as follows.
%
For mutations, \system essentially performs two types of operations on a selected transition $\mathcal{R}$ as discussed below. 

%\syed{Please connect the following discussion with insight I3. The connection is loose in the current write-up. Our mutations are of two types and they have two goals: state-aware and property-driven.}
\noindent\ding{111} \textbf{M1: Mutating the observation of a transition.} 

\system{} alters the observation $(\alpha/\gamma)$ of $\mathcal{R}$,  i.e., alters either the input $\alpha$ or the output $\gamma$ or both based on the input and output in trace skeleton \tracesup{a} when the execution reaches at $q_c$. 

%The goal of this mutation kind is to either (i) mutate the input and output message of a transition at state $q_c$ to satisfy an input symbol in the given test skeleton $\pi^{a}$, or 
%(ii) mutate the input message to observe a deviation, i.e., a behavior in the target implementation \pimp different from what the guiding PSM suggests, such as acceptance of a prohibited message at a certain state.
%(ii) mutate the input message to observe a deviation, such as the target implementation \pimp accepting a prohibited message at a specific state, differing from what the guiding PSM suggests.

%
% The goal of this mutation kind is to either (i) mutate the input and output message of a transition at state $q_c$ to satisfy an input symbol in the given test skeleton $\pi^{a}$, or (ii) mutate the input message to observe any deviation, i.e., a behavior in the target implementation \pimp different from what the guiding PSM suggests, such as acceptance of a prohibited message at a certain state.
%
%Since we mutate the observation of a defined transition from the guiding FSM at a specific state, we ensure that only certain input messages, which are likely to be accepted by the target implementation at that state, are mutated. This contrasts with traditional fuzzers that randomly select messages to mutate without considering the device's current state.  
%
%We consider the first objective when we generate a concrete trace from a given trace skeleton $\pi^{a}$ (\S\ref{sec:tracebuilder:trace_generation}). 
%At a certain state $q_c$, suppose we require a specific input $\alpha'$ and output $\gamma'$ according to the given test skeleton, and it is not prescribed by the guiding PSM $\mathcal{M}$ at $q_c$. 

If the trace skeleton \tracesup{a} requires input $\alpha'$ and output $\gamma'$ at state $q_c$ but the guiding PSM $\mathcal{M}$ does not have $\alpha'/\gamma'$at $q_c$, to ensure the generated trace conforms with \tracesup{a}, we mutate the transition $\mathcal{R}$ in $\mathcal{M}$ with $\alpha'$ to obtain input $\alpha'$ and output $\gamma'$, i.e., $\mathcal{R}'(q_c, \alpha', \gamma', q_n)$. For example, in Figure 1, suppose at state $q_5$ if we require output \footnotesize\textsc{GUTI\_ reallocation \_complete}\normalsize\xspace for input
\footnotesize\textsc{GUTI\_ reallocation \_command: Replay ==1}\normalsize\xspace according to the test skeleton. However, since it is not prescribed at state $q_5$, we mutate the transition with observation $a_{gc}$ (with input \footnotesize\textsc{GUTI\_ reallocation \_command}\normalsize\xspace) to obtain input \footnotesize\textsc{GUTI\_ reallocation \_command: Replay == 1}\normalsize\xspace and output \footnotesize\textsc{GUTI\_ reallocation \_complete}\normalsize\xspace.
This mutation strategy is required to generate traces that satisfy a given test skeleton and test for violations of its associated security property.

\input{tables/mutation_operation}

%We consider the second objective when we are instantiating the wildcard characters of a test skeleton $\pi^{a}$, and decide to test with a mutated version of an input message to detect any deviation from the PSM that can lead to a security property violation. 

On the other hand, if \tracesup{a} has a wildcard character at state $q_c$, \system{} instantiates the wildcard character with a mutated version of an input message $\alpha$ to detect any deviation from the PSM that can lead to a security property violation. 
To increase the likelihood of a mutated message being accepted by a practical protocol implementation, \system{} considers the semantic meaning of the input message. It performs one of the six semantic operations. We summarize these operations with examples in Table \ref{tab:mutation_ops_m1}. These operations consider the semantics of the message fields, their defined values and ranges according to the protocol specification, and overall message semantics (e.g., plaintext or replayed version). As an example, in Figure \ref{fig:mutation_kind_example}(i), consider a mutation of the transition with observation $a_{ap}$ (with input \footnotesize\textsc{attach\_ accept: integrity == 0 \& cipher == 0 \& security\_ header \_ type == 0}\normalsize\xspace, marked blue) at state $q_1$. If we perform \textbf{OP2} operation and change the value of the \footnotesize\textsc{security\_ header \_ type}\normalsize\xspace  field to a prohibited value 4, we obtain the mutated message $a_{ap}'$ with input \footnotesize\textsc{attach\_ accept: integrity == 0 \& cipher == 0 \& security\_ header \_ type == 4}\normalsize\xspace. If the target implementation accepts this mutated message, we obtain a response (e.g., \footnotesize\textsc{attach\_ complete}\normalsize\xspace), which deviates from the guiding PSM.

% \updated{
% Furthermore, to incorporate mutations that have semantic meaning, we consider performing certain operations that alter the field value or a general property of the original message. To mutate any input message $\alpha$, we perform any of the six operators mentioned in Table \ref{tab:mutation_ops_m1}. After applying any of the operators, we obtain a mutated input message, and hence a mutated observation over a transition. 
% }

% \updated{
% For operation \textbf{OP1}, we select a particular message field and set it to a random value within its defined range according to the protocol specification. For example, in a \connectionreq message in BLE, we can set the 5-bit \textit{Hop} field to a value between 5 and 16. For operation \textbf{OP2}, we change the value of a particular field to a prohibited or reserved value. For instance, in a \connectionreq message in BLE, we can set the 5-bit \textit{Hop} field to a value greater than the maximum defined range of 16. This operation also includes setting incorrect key values in specific messages, such as sending a \keyexchange message in BLE with incorrect key values. For operation \textbf{OP3}, we set a field to its boundary values. For example, we can mutate a \connectionreq message by setting the \textit{channelMap} field to 0. For operation \textbf{OP4}, we send a plaintext version of a message that is typically expected to be integrity-protected and/or ciphered. For example, we can send an \attachacc message in 4G LTE in plaintext. For operation \textbf{OP5}, we combine multiple operations from \textbf{OP1} through \textbf{OP4}, allowing for the mutation of multiple fields simultaneously. This approach can be particularly useful for uncovering complex bugs. For example, we can send an \authreq message in 4G LTE with the separation bit set to 0 and the security header type set to 3. Finally, for operation \textbf{OP6}, we replay a previously captured instance of the message we are mutating. For example, we can send a replayed \smcmd message in 4G LTE after the NAS security context has been established. These mutation operations are designed to introduce meaningful variations in the input messages, with the goal of uncovering security vulnerabilities and unexpected deviations in protocol behavior.
% } 
%\syed{Incorporate the examples into the table in a new column.}
\begin{figure}[htbp]
\centering
\resizebox{0.5\linewidth}{!}{%
\begin{tikzpicture}[>=stealth',bend angle=45,auto]

\tikzstyle{state}=[circle,thick,draw=black!100,fill=white!20,minimum size=1.2cm,text width=1.5cm,align=center,inner sep=0pt,line width=1mm]
\tikzstyle{edgeLabel}=[pos=0.5,text centered,text width=5cm,font={\sffamily\fontGuidingFSMFig}];  % Adjusted font size here
\tikzset{every loop/.style={min distance=1mm,looseness=3}}

\begin{scope}[->,node distance=4.2cm,yshift=0mm, xshift=-135mm, local bounding box=a_nodes]
% First net
\node [state, name=q0] {\fontGuidingFSMFig q0};
\node [state, name=q1, right of=q0, yshift=0mm] {\fontGuidingFSMFig q1};
\node [state, name=q2, right of=q1, yshift=0mm] {\fontGuidingFSMFig q2};
\node [state, name=q3, right of=q2, yshift=0mm] {\fontGuidingFSMFig q3};
\node [state, name=q4, right of=q3, yshift=0mm] {\fontGuidingFSMFig q4};
\node [state, name=q5, right of=q4, yshift=0mm] {\fontGuidingFSMFig q5};

\path[every node/.style={font=\sffamily\Large,inner sep=0pt}]
    (q0) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ea}$} (q1)
    (q1) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ar}$} (q2)

    % (q1) edge[red, loop above, out=120, in=60, looseness=5, yshift=20mm,  densely dashed, line width=1mm] node[edgeLabel, line width=1mm] {\fontGuidingFSMFig$a_{ac'}$} (q1)

    (q1) edge[blue, loop below, out=125, in=55, looseness=6, line width=1mm] node[edgeLabel, yshift=10mm, xshift=0mm] {\fontGuidingFSMFig$a_{ap}$} (q1)

    
    (q2) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{sm}$} (q3)
    (q3) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{rs}$} (q4)
    (q3) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=3mm, xshift=0mm, line width=1mm] {$a_{id}$} (q3)

    (q3) edge[bend right=-60, line width=1mm] node[edgeLabel,yshift=-2mm,xshift=2mm] {\fontGuidingFSMFig$a_{dr}$} (q0)
    (q5) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gc}$} (q5)
    (q5) edge[loop below, out=-120, in=-60, looseness=5, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gr}$} (q5)

    % new add for mutation - ridwan
    (q1) edge[red, loop below, out=-125, in=-55, looseness=6, densely dashed, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{ap'}$} (q1)

    % (q1) edge[red, bend right=-40, densely dashed, line width=1mm] node[edgeLabel,yshift=2mm,xshift=-8mm] {\fontGuidingFSMFig$a_{ac'}$} (q5)
    
    
    (q4) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ac}$} (q5);
\end{scope}
\end{tikzpicture}
    }
    
    % \vspace{0.5cm}
    \textbf{(i) Mutation Kind $\mathbf{M1}$}
    
    % \vspace{1cm}
    
    \resizebox{0.5\linewidth}{!}{
    \begin{tikzpicture}[>=stealth',bend angle=45,auto]
    
    \tikzstyle{state}=[circle,thick,draw=black!100,fill=white!20,minimum size=1.2cm,text width=1.5cm,align=center,inner sep=0pt,line width=1mm]
    \tikzstyle{edgeLabel}=[pos=0.5,text centered,text width=5cm,font={\sffamily\fontGuidingFSMFig}];  % Adjusted font size here
    \tikzset{every loop/.style={min distance=1mm,looseness=3}}
    
    \begin{scope}[->,node distance=4.2cm,yshift=0mm, xshift=-135mm, local bounding box=a_nodes]
    % First net
    \node [state, name=q0] {\fontGuidingFSMFig q0};
    \node [state, name=q1, right of=q0, yshift=0mm] {\fontGuidingFSMFig q1};
    \node [state, name=q2, right of=q1, yshift=0mm] {\fontGuidingFSMFig q2};
    \node [state, name=q3, right of=q2, yshift=0mm] {\fontGuidingFSMFig q3};
    \node [state, name=q4, right of=q3, yshift=0mm] {\fontGuidingFSMFig q4};
    \node [state, name=q5, right of=q4, yshift=0mm] {\fontGuidingFSMFig q5};
    
    \path[every node/.style={font=\sffamily\Large,inner sep=0pt}]
        (q0) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ea}$} (q1)
        (q1) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ar}$} (q2)
    
        % (q1) edge[red, loop above, out=120, in=60, looseness=5, yshift=20mm,  densely dashed, line width=1mm] node[edgeLabel, line width=1mm] {\fontGuidingFSMFig$a_{ac'}$} (q1)
    
        (q1) edge[blue, loop below, out=125, in=55, looseness=6,line width=1mm] node[edgeLabel, yshift=10mm, xshift=0mm] {\fontGuidingFSMFig$a_{ap}$} (q1)
    
        
        (q2) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{sm}$} (q3)
        (q3) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{rs}$} (q4)
        (q3) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=3mm, xshift=0mm, line width=1mm] {$a_{id}$} (q3)
    
        (q3) edge[bend right=-60, line width=1mm] node[edgeLabel,yshift=-3mm,xshift=-9mm] {\fontGuidingFSMFig$a_{dr}$} (q0)
        (q5) edge[loop above, out=120, in=60, looseness=5, line width=1mm] node[edgeLabel, yshift=1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gc}$} (q5)
        (q5) edge[loop below, out=-120, in=-60, looseness=5, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gr}$} (q5)
    
        % new add for mutation - ridwan
        % (q5) edge[red, loop below, out=-135, in=-45, looseness=10, densely dashed, line width=1mm] node[edgeLabel, yshift=-1mm, xshift=0mm] {\fontGuidingFSMFig$a_{gr'}$} (q5)
    
        (q1) edge[red, bend right=-40, densely dashed, line width=1mm] node[edgeLabel,yshift=2mm,xshift=-8mm] {\fontGuidingFSMFig$a_{ap}$} (q5)
        
        
        (q4) edge[bend right=0, line width=1mm] node[edgeLabel,yshift=1mm,xshift=0mm] {\fontGuidingFSMFig$a_{ac}$} (q5);
    \end{scope}
    \end{tikzpicture}
    }
    
    % \vspace{0.5cm}
    \textbf{(ii) Mutation Kind $\mathbf{M2}$}
    
    
    \caption{Two types of Mutations M1 and M2. The transition labels are presented in Table \ref{tab:ble_running_example_table}.}
    \label{fig:mutation_kind_example}
    \vspace{-0.2cm}

\end{figure}

\noindent\ding{111} \textbf{M2: Mutating the destination state of a transition.} 

In this case, we alter the destination state $q_n$ of a selected transition $\mathcal{R}$ $(q_c, \alpha, \gamma, q_n)$. The goal of this kind of mutation is to test whether the input message $\alpha$ at state $q_c$ leads to a state $q_m$ different than what is expected  by the guiding PSM (in this case $q_n$), which in turn can lead to an observable deviation or security property violation. This kind of mutation enables \system to detect certain bypass attacks (e.g., check whether any intermediate step can be bypassed to reach a secure state). 

% \system generates an instantiated trace that tests whether input message $\alpha$ at state $q_c$ leads to a state $q_m$ different than what is expected (in this case $q_n$) by the guiding PSM, which in turn can lead to an observable deviation or security property violation. This kind of mutation also enables \system to detect certain bypass attacks (e.g., check whether any intermediate step can be bypassed to reach a secure state). 

As an example, in Figure \ref{fig:mutation_kind_example}(ii), suppose we perform mutation over the transition with observation $a_{ac'}$ at state $q_1$ (marked blue). We can perform a mutation over the next state $q_2$ of the transition by changing the next state of the transition to $q_5$. This mutation would generate an instantiated trace that tests whether the target implementation incorrectly reaches state $q_5$ if a plaintext \attachacc is fed at state $q_1$.


\vspace{-0.3cm}
\subsection{Instantiated Trace Generation}\label{sec:tracebuilder:trace_generation}
%\textcolor{blue}{Finally, for a given trace skeleton \tracesup{a}, the challenge is to design an automatic approach to generate test traces $\gamma$ that would (1) satisfy the regular expression $\sigma_i$, (2) align with the guiding PSM $\mathcal{M}$, (3) ensure that each generated trace $\gamma$ require at most $\mu$ mutations on $\mathcal{M}$, and (4) maintain a maximum length of $\lambda$.} 

Given a test skeleton \tracesup{a} representing violation of a property $\phi \in \Phi$, a guiding PSM $\mathcal{M}$, a mutation budget $\mu$ and a length budget $\lambda$, we leverage insight \textbf{I2} and solve the problem of generating instantiated traces by combining the solutions of overlapping subproblems. For this, we formulate a dynamic programming problem as follows.

%textcolor{red}{originating from the destination state of a trace in $\mathcal{M}$ to a particular state in the trace.} \syed{Hard to understand} For this, we formulate a dynamic programming algorithm as follows.

% \begin{tcolorbox}
$\mathbf{\mathcal{G}(\mathcal{M}, \tracesup{a}, q_c, \mu, \lambda)}$: \emph{At any state $\mathsf{q}_c \in \mathcal{Q}$ of a guiding PSM $\mathcal{M}$, we want to craft a set of instantiated traces $\mathcal{T}$, where each instantiated trace (i) satisfies the test skeleton \tracesup{a}, (ii) is the outcome of a maximum of $\mu$ mutations applied on any trace in the guiding PSM $\mathcal{M}$ and (iii) is within a maximum length $\lambda$.}     
% \end{tcolorbox}

We use $\mathcal{G}(\mathcal{M}, \tracesup{a}, q_c, \mu, \lambda)$ to denote the problem which we can solve by leveraging the solution to its \emph{overlapping subproblems}. Consider we are at state $q_i$ of our guiding PSM $\mathcal{M}$ and we need to satisfy the $j^{th}$ observation $l_j$ = $(\alpha_j/\gamma_j)$ of the test skeleton \tracesup{a} (i.e, the test skeleton up to input symbol $l_{j-1}$ has been satisfied) and the next wildcard character in \tracesup{a} is $l_k$. Also, consider at $q_i$ the remaining mutation budget is $\mu_{i}$ and the remaining length budget is $\lambda_i$. For this problem, we consider the following four cases, where we formulate subproblems and prepend observations according to the following case.

\textbf{Case I.} If there is a transition $\mathcal{R}(q_i, \alpha, \gamma, q_m)$ at state $q_i$ whose observation satisfies $l_j$, \dpalgo can leverage solutions from the destination state $q_m$ that satisfies \tracesup{a} from observation $l_{j+1}$, with mutation budget $\mu_{i}$ and length budget $\lambda_i - 1$. \dpalgo prepends $l_j$ to the instantiated traces being generated from the subproblem. Since it places an observation ($l_j$) in the instantiated trace, it uses length budget $\lambda_i - 1$ to formulate the subproblem.

\textbf{Case II.} If there is no transition whose observation satisfies $l_j$, \dpalgo can consume a mutation to mutate the transition for $\alpha_j$ (the input message of observation $l_j$) to place observation $l_j$ in the instantiated trace, using mutation kind \textbf{M1}. Again \dpalgo leverages traces from the destination state of the transition $q_m$ that satisfies \tracesup{a} from observation $l_{j+1}$, with length budget $\lambda_i - 1$ but with mutation budget $\mu_i - 1$ since it consumed a mutation to place $l_j$. \dpalgo prepends $l_j$ to the obtained instantiated traces from the subproblem.

\textbf{Case III.} If there is a transition $\mathcal{R}(q_i, \alpha, \gamma, q_m)$ at state $q_i$ whose observation $(\alpha/\gamma)$ satisfies wildcard character element $l_k$, \dpalgo leverages solutions from the destination state $q_m$ that satisfies \tracesup{a} from observation $l_{j}$ with mutation budget $\mu_{i}$ and length budget $\lambda_i - 1$. It prepends observation $(\alpha/\gamma)$ to the obtained instantiated traces from the subproblem.

\textbf{Case IV.} Finally, for any transition $\mathcal{R}(q_i, \alpha, \gamma, q_m)$ at state $q_i$, \dpalgo can mutate the transition's observation and place a mutated observation $(\alpha/\gamma)_m$ using mutation kind \textbf{M1}. \dpalgo can leverage solutions from the destination state $q_m$ that satisfies \tracesup{a} from observation $l_{j}$ with length budget $\lambda_i - 1$ and also mutation budget $\mu_i - 1$ since we perform a mutation. It prepends the mutated observation $(\alpha/\gamma)_m$ to the obtained instantiated traces from the subproblem. Note that, we only place a \textit{mutation marker} in this case. This marker would be resolved by the \textit{mutation resolver} component of \dispatcher (\S\ref{sec:trace_dispatcher}) later on though operating on the input message $\alpha$ using one of the six operations described in \S\ref{sec:tracebuilder:mutation}. Note that, by placing various mutated message in place of the mutation marker, we can generate multiple traces to test OTA. 

Furthermore, for each case, \dpalgo may also consider mutating the destination state of the selected transition (mutation kind \textbf{M2}). In that case, \dpalgo mutates the destination state to another state $q_{mut}$ and formulates the subproblem from state $q_{mut}$ with mutation budget $\mu - 1$. \dpalgo will terminate if either \tracesup{a} is satisfied or it runs out of mutation or length budget.




%A detailed algorithm for \dpalgo is provided in Algorithm \ref{algo:tracebuilder} in Appendix and the base and recursive steps of the proposed dynamic programming algorithm are discussed in Appendix. 

%\syed{Need to discuss the cases of DP algorithm briefly here. For example, what happens if the j-th position of the RE is a literal/kleene star and that matches/doesn't match with the i-th symbol in a trace in M. When there is no match, the algorithm introduces mutations, i.e., mutation marker. The previous paragraph should be revised according to this suggestion. Also, when we say M in this algorithm, it is actually a trace in M in each iteration. If we can make this discussion simple, we do not need to introduce forward transition and allowed transition discussed in Appendix.} 


% Like any dynamic programming Algorithm, Tracebuilder also has a base case and a recursive step. \dpalgo considers mutations on the given guiding PSM \pimp to generate test traces. We first discuss the extraction of our guiding PSM. Then we discuss our notion of \textit{mutation} in detail. Finally we discuss the base case and recursive steps of \dpalgo.
%\input{algorithms/tracebuilder}





% For mutation kind \textbf{M1}, for each message type, we consider a \textit{mutation pool} which is a set of mutated variations of that message type (e.g. for \textsl{enc\_pause\_req} we consider \textsl{enc\_pause\_req: integrity == 0 \& replay == 0} and \textsl{enc\_pause\_req: integrity == 1 \& replay == 1} ). We consider a message from this mutation pool whenever a message needs to be mutated. Also, for mutation kind \textbf{M2}, for each state $q_c$, we consider the mutated next state $q_m$ among a given set of states. These sets and mutation pool can also be considered input to \system.

%  Proteus randomly applies one perturbation from a pool of available strategies. For example, it replaces an integrity protected message with a plaintext or a replayed one, or varies security sensitive fields (e.g., identity type in Identity Request, security header type etc.) in messages, and their combination thereof (e.g., plaintext identity request with identity type 3 (TMSI) and security header type 1).

% 



==> sections/8_tracedispatcher.tex <==
\section{\dispatcher: Execution of Generated Traces and Detection of Flaws}
\label{sec:trace_dispatcher}



Once \system obtains a set of test traces $\mathcal{T}$ from \dpalgo, the \dispatcher component of \system iteratively selects traces from $\mathcal{T}$ to test over the air against the target implementation (\pimp). The \dispatcher runs for $t$ iterations, where $t$ corresponds to the testing budget regarding the maximum number of traces we can test or the number of traces one can test OTA within a fixed time. 

At each iteration, the \textit{scheduler} component of \dispatcher follows a selection criteria to select a trace $\gamma$ in $\mathcal{T}$ to test. \system attempts to find as many violations as possible within the given testing budget. As such, it adopts a selection technique to select test traces targetting as much state coverage (w.r.t the guiding PSM) and code coverage as quickly as possible. Once a test trace $\gamma$ is selected, the \textit{mutation resolver} component of \dispatcher then resolves any mutation marker (\S\ref{sec:tracebuilder:recursivestep}) in $\gamma$, placing a concrete observation instead of the marker and obtaining a concrete trace $\gamma_c$. Next, the \textit{adapter} component of \dispatcher converts the abstract input symbols in the test trace into concrete messages and sends them OTA to the target implementation. The \textit{adapter} also receives the concrete response and converts to an abstract output symbol within \system s' output alphabet. Finally, the \textit{observer} component of \dispatcher analyzes the response checks whether \pimp follows $\gamma_c$. \textit{Observer} detects whether any deviation from the guiding PSM or a security property violation has occurred, and if so, reports it. It also records some relevant information that are used by the \textit{scheduler} to schedule future test traces. We now discuss the different components of \dispatcher in detail.

%\noindent\textbf{Adapter.} The input symbols in the traces generated by \system and scheduled to be tested OTA are abstract. The \textit{adapter} component converts the abstract input symbols in a trace into concrete messages. Each abstract input symbol in the input alphabet $\Sigma$ mentions a message type and also mentions associated predicates. The \textit{adapter} generates a concrete message of the specified message type satisfying all specified predicates accordingly. The \textit{adapter} then executes each concrete message in order and collects the response from the target implementation. Upon receiving a concrete response message the adapter converts it to an abstract output symbol in the output alphabet $\Lambda$ which can be interpreted by the \textit{observer} component of \dispatcher.

\noindent\textbf{Scheduler.} In each testing iteration, the \textit{scheduler} component of \dispatcher first chooses a property $\phi \in \Phi$ to test and then selects a test trace $\gamma$ associated with $\phi$. The \textit{scheduler} employs weighted random sampling to select a property $\phi$ from $\Phi$. The \textit{scheduler} determines the weight of each property by determining the no. of distinct states covered by all concrete test traces associated with $\phi$ w.r.t. the guiding PSM and taking their average. This scheme favors properties whose test traces cover more states within the guiding PSM.


% Each trace $\gamma$ obtained from the generated trace set $\mathcal{T}$ can be classified into one of these two classes: (ii) \textit{concrete trace} if all the observations in the trace are concrete input symbols, with no mutation markers. A protocol adapter can directly translate the sequence of input symbols for this kind of trace to create concrete messages and dispatch OTA and (ii) \textit{non-concrete trace} which has at least one observation with a mutation marker (i.e., observation of the form ${(\alpha/\beta)}$ in discussed in Section \ref{sec:tracebuilder:recursivestep}). The observations with the mutation markers need to be \textit{resolved} by \dispatcher and converted to a concrete input symbol. Note that a concrete trace is obtained from a non-concrete trace if we resolve all its mutation markers, and as such, one can generate multiple concrete traces from a non-concrete trace.

Note that there are two kinds of traces generated by \dpalgo: (a) Traces with no observation with mutation markers (\S\ref{sec:tracebuilder:mutation}). \textcolor{red}{All input symbols in this kind of trace are within the input alphabet} \syed{This sentence is not clear.} and can be directly translated into a concrete message by the \textit{adapter} and (b) Traces with at least one observation mutation marker. The observations with the mutation markers need are resolved by the \textit{mutation resolver} component of \dispatcher and converted to an input symbol within the input alphabet $\Sigma$. Note that a type (a) trace is obtained from a type (b) trace if we resolve all its mutation markers, and as such, one can generate multiple type (a) traces from a type (b) trace. \syed{Need to simplify this discussion}

Once a property $\phi$ is selected, The \textit{scheduler} chooses a trace $\gamma$ for testing from all associated traces of $\phi$. It first randomly decides whether to test a type (a) or a type (b) trace. Since type (b) traces test with mutated input symbols representing attacker crafted messages, these traces have more potential to trigger property violations. As such, we pick traces of type (b) with more probability.

If \textit{scheduler} chooses a type (a) trace, it randomly picks a test trace to test. For type (b) traces, the \textit{scheduler} prioritizes traces that are either untested or tested the least. Test traces triggering known deviations are also prioritized, as they can lead \pimp to an inconsistent state where \system may find more property violations. However, if a deviation causes \pimp to become unresponsive, \dispatcher is less inclined to test that trace, as an unresponsive \pimp would not lead to any new property violation. Consequently, the \textit{scheduler} selects a type (b) trace based on three factors: the frequency of selection ($f$) of $\gamma$, the number of deviations covered by $\gamma$ ($d$), and the instances where $\gamma$ rendered \pimp unresponsive ($u$). Finally, \dispatcher selects the test trace with the minimum score ($p = f - d + u$), randomly choosing one if multiple test traces share the minimum score.

\noindent\textbf{Mutation Resolver.}  For each type (b) trace, we must resolve all observations with mutation markers (i.e., observations of the form ${(\alpha/\beta)}_m$ from \dpalgo). Given an observation $(\alpha/\beta)$ to mutate, we focus on mutating input symbol $\alpha$ to $\alpha_m$ where $\alpha_m$ is wihtin the input alphabet $\Sigma$. Any response to $\alpha_m$ is deemed acceptable from the attacker's perspective (i.e., we need not consider any particular value for $\beta_m$).

Consider input symbol $\alpha$ comprises of message type $m$ and predicates $f_1, f_2, \ldots, f_p$. We maintain a \textit{mutation pool} for each message type $m$, containing various combinations of predicates. Each message in the mutation pool is within the input alphabet $\Sigma$ and can be translated into a concrete message by the \textit{adapter}. For instance, in LTE, for the \smcmd message type, we include mutations such as \smcmdreplayfull (indicating a replayed message) and \smcmdplaineiazero (indicating a plaintext message with EIA0) and so on. 

For mutations, we consider variations such as plaintext and replayed versions of integrity-protected message types and changes in the security header type for any message. Additionally, we can also consider any security-sensitive field using domain-specific knowledge (e.g., in LTE, we consider the \idtype field of the \idreq message).

\noindent\textbf{Observer.} Given a trace $\gamma_c = \alpha_1/\beta_1, \alpha_2/\beta_2, \ldots, \alpha_k/\beta_k$ with all mutation markers resolved to test by the \textit{scheduler}, the \textit{observer} observes the response of \pimp $r_1, r_2, \ldots, r_k$. It also obtains the reference behavior $\tau_1,\tau_2,\ldots,\tau_k$ to the input sequence w.r.t. the guiding PSM. If any response message $r_i$ does not comply with the reference behavior $\tau_i$, we consider it as a \textit{deviation}. In case of deviations, the \textit{observer} also checks whether \pimp violates any of the input security properties $\Phi$, and if so, it reports the violation. 

In addition, the \textit{observer} records the following information while testing and observing responses, which the \textit{scheduler} component of \dispatcher uses during the selection of a test trace in future iterations: (i) Any deviation observed when testing a message of type $m$ at a particular protocol state $s$, (ii) The frequency of selection of any non-concrete trace. (iii) How many times a trace with any mutation marker rendered \pimp unresponsive. To determine unresponsiveness, the \textit{observer} identifies the final protocol state $s_f$ according to the guiding PSM for each test trace. It then executes a message $i_f$ OTA (Over-The-Air) expected to elicit a valid output message $o_f$. If \pimp does respond with any reply message, it is deemed unresponsive. (iv) The number of times \dispatcher mutated each message type $m$ to resolve any trace with mutation markers and (v) Violation of any property $\phi \in \Phi$. The \textit{scheduler} removes $\phi$ from $\Phi$ if a violation of $\phi$ is observed, thus eliminating all test traces associated with $\phi$ (i.e. test traces generated with trace skeletons that violate $\phi$).
